Relevance Feedback with Brain Signals

The Relevance Feedback (RF) process relies on accurate and real-time relevance estimation of feedback documents to improve retrieval performance. Since collecting explicit relevance annotations imposes an extra burden on the user, extensive studies have explored using pseudo-relevance signals and implicit feedback signals as substitutes. However, such signals are indirect indicators of relevance and suffer from complex search scenarios where user interactions are absent or biased. Recently, the advances in portable and high-precision brain-computer interface (BCI) devices have shown the possibility to monitor user's brain activities during search process. Brain signals can directly reflect user's psychological responses to search results and thus it can act as additional and unbiased RF signals. To explore the effectiveness of brain signals in the context of RF, we propose a novel RF framework that combines BCI-based relevance feedback with pseudo-relevance signals and implicit signals to improve the performance of document re-ranking. The experimental results on the user study dataset show that incorporating brain signals leads to significant performance improvement in our RF framework. Besides, we observe that brain signals perform particularly well in several hard search scenarios, especially when implicit signals as feedback are missing or noisy. This reveals when and how to exploit brain signals in the context of RF.

==> Cover/AE.tex <==
\noindent\textbf{Responses to AE:}
\vspace{0.1cm}

\vspace{0.2cm}
\textbf{<AE.1>} \textit{The details of the user study are not clear enough.}

\textbf{Response:} Thanks for your concerns. 
We revise Section~\ref{3} to include more details of the main task procedures, the stimuli presentation, and the annotation process in the user study. 
We also add Section~\ref{Interface of the lab study} in the appendix to provide examples and screenshots of the main task. 
Additionally, our github repository~(https://github.com/THUIR/Brain-Relevance-Feedback) is updated with the code and instructions of the user study system for a better understanding and replication of the data collection procedures study.

\textbf{Revision:} \textcolor{blue}{Please refer to Section~\ref{3} and Section~\ref{Interface of the lab study}.}

\vspace{0.2cm}
\textbf{<AE.2>} \textit{There are a few concerns about the setting of this user study such as privacy, participants, and EEG availability.}

\textbf{Response:} To address these concerns, we add more explanations and discussions on privacy~(detailed in <R1.2>), participants~(detailed in <R2.2>), and EEG availability~(detailed in <R1.2>).

\textbf{Revision:} \textcolor{blue}{Please refer to Section~\ref{2.3} and Section~\ref{6.2} for revisions on the discussions about the privacy issue, EEG availability issue, and discussions of applications. 
Kindly refer to Section~\ref{3} Line~\lineref{l3.1} for the discussion regarding the number of participants and statistical power analysis.}

\vspace{0.2cm}
\textbf{<AE.3>} \textit{The motivations of using the brain signal are not clear. Authors are suggested to clearly state the reason of why it is necessary to study brain signal in retrieval task.}

\textbf{Response:} Thanks for your concerns.
We clarify the motivation of our study in Section~\ref{1}, and we also add some discussion on the comparison of conventional signals and application scenarios in Section~\ref{6.2}.
Traditionally, implicit signals~(e.g., click, dwell time) are usually considered more reliable than pseudo-relevance signals for RF.
Nevertheless, implicit signals are indirect probes of relevance inferred from user’s behaviors and thus are often biased and inaccurate~\cite{45lu2018between}. 
While existing research attempts to mitigate these biases by utilizing additional signals such as eye-tracking and mouse movement, practical experience has revealed that these indirect signals still bring biases. 
For instance, the credibility of eye-tracking signals is limited as gazing at a document can not necessarily guarantee that its content is genuinely relevant~\cite{mao2014estimating}.
Unlike existing signals, brain signals directly reflect a user’s psychological activities and are therefore not subject to the inherent bias of user behaviors.
Therefore, we aim to explore the effect of brain signals in the context of RF~(including IRF and RRF).
Furthermore, we investigate search scenarios in which brain signals have a pronounced significance, shedding light on viable scenarios for BCI applications within IR.

\textbf{Revision:} \textcolor{blue}{Please refer to Section~\ref{1} Line~\lineref{1.motivation.1}, Section~\ref{1} Line~\lineref{1.motivation.2} and Section~\ref{6.2}.}

\vspace{0.2cm}
\textbf{<AE.4>} \textit{The experiment needs to be improved by giving reasonable explanations to the results and may include more scenarios of different biases.}

\textbf{Response 1:} 
Thanks for your comments. 
We clarify Section~\ref{5.1} with a sensitivity analysis and more deicussions about the brain decoding experiment.
We also clarify Section~\ref{5.3} with a more detailed explanation of combination parameter analysis and add a case study in Section~\ref{Case studies} to illustrate the effect of RF, especially when in combination with brain signals.
% We also study the effect of the confounders~(as detailed in <R2.4>)~(as detailed in <R2.4>) and discuss other bias in Section~\ref{6.2}~(as detailed in <R3.7>).

\textbf{Response 2:} We acknowledge that there are many types of confounding factors and biases existing in user’s search behaviors. 
Due to the limited resources, we cannot do separate lab studies to evaluate and analyze each type of them in this paper, but we conducted a statistical causal analysis on several well-recognized factors, including individual differences, the display type of the documents, the task rank, the documents rank, and the word number in the documents. 
Our analysis shows that the relevance of documents has a significant and detectable effect on participants’ brain signals even if we take all these confounders into account. 
Please refer to <R2.4> and <R3.7> for more details. 

\textbf{Revision:} \textcolor{blue}{Please refer to Section~\ref{5.1} and Section~\ref{5.3} for the clarifications on the experimental results. Kindly refer to Section~\ref{A.2} for the statistcial casual analysis.}

\vspace{0.2cm}
\textbf{<AE.5>} \textit{The presentation of this paper is suggested to be improved.}

\textbf{Response:} 
Thanks for your comments.
We revised all issues noted by the reviewers, and polished the whole paper to improve its readability.
To be more specific, we have added Section~\ref{Interface of the lab study} to clarify the search interface used in the user study process and included a case study in Section~\ref{Case studies} to illustrate the RF cases from our research. 
Additionally, we add an algorithm in Section~\ref{5.0} to simplify the understanding of the RF pipeline.
We also restructured Section~\ref{6} to address concerns and questions related to motivation, privacy issues, EEG availability, application scenarios, and other related topics. 
Moreover, we go through the whole paper to improve the representation and fix the language issues.



==> Cover/Cover_letter_ziyi.tex <==
\newpage
\thispagestyle{empty}
\large

Dear Editors and the Review Team,

\vspace{0.2cm}
We would like to thank you for your constructive comments and advice on our manuscript titled:%\smallskip

% \centering
\textbf{Relevance Feedback with Brain Signals}
% \smallskip

% \raggedright
We have carefully considered the suggestions from AEs and reviewers for our manuscript. 
All changes are summarized below, and the updated manuscript is attached to this document.
The summarization of the revisions we have made to this manuscript includes:

\begin{itemize}
    \item[$\bullet$ <S1>] Revise the manuscript to a include more detailed description of the user study and RF experiments.
    \begin{itemize}
        \item[- <S1.1>] We add more explanations to the user study procedures in Section~\ref{3} and add Section~\ref{Interface of the lab study} in the appendix to provide examples and screenshots of the main task.
        \item[- <S1.2>] We add Section~\ref{5.0} and Algorithm~\ref{algorithm:pipeline} to explain the training and evaluation pipeline of RF, as well as the data-splitting protocols.
        \item[- <S1.3>] We add Section~\ref{Case studies} to illustrate the necessity of exploiting brain signals to improve search performance with a case study.
    \end{itemize}
    \item[$\bullet$ <S2>] We revise Section~\ref{2}, Section~\ref{3}, and Section~\ref{6} to address the privacy concerns, participants, EEG availability, etc.
    \item[$\bullet$ <S3>] Revise the manuscript to make the experimental results more comprehensive.
    \begin{itemize}
        \item[- <S3.1>] We add additional baselines BM25 in Section~\ref{5} and a statistical study concerning the confounders involved in our research in Section~\ref{A.2}.
        \item[- <S3.2>] We clarify the experimental settings and experimental results regarding different selections of the combination parameters experiment.   
        \item[- <S3.3>] We add a sensitive analysis about the EEG preprocessing settings in Section~\ref{Sensitivity analysis}, which offers guidance for neurological preprocessing in real-time RF scenarios.  
    \end{itemize}
    \item[$\bullet$ <S4>] We add some discussions regarding the insights of our paper, the role of brain signals, the comparison with existing signals~(such as eye-tracking), and the application scenarios in Section~\ref{1}, and Section~\ref{6}.
    \item[$\bullet$ <S5>] We also tone down some interpretations of the manuscript, improve the figures and tables, and polish the whole paper to improve its readability.
    
\end{itemize}

The detailed responses and revisions for each reviewer are given below.
Note that the review team's comments are \textit{italicized}, and our responses and manuscript revisions begin with \textbf{``Response''} and \textbf{``Revisions''}, respectively.
Each review is assigned a unique identifier. 
The abbreviation AE denotes Associate Editor, R1 denotes Reviewer 1, R2 denotes Reviewer 2, and R3 denotes Reviewer 3. 
The $j^{th}$ comment from Associate Editor and Reviewer $i$ is indexed as <AE.j> and <Ri.j>, respectively.

Besides, in the manuscript, \textcolor{blue}{all revisions are highlighted in blue.}
We thank the editors and reviewers again for the constructive comments. 

\vspace{0.3cm}
Best regards,

Ziyi Ye, Xiaohui Xie, Qingyao Ai, Yiqun Liu, Zhihong Wang, Weihang Su, Min Zhang

\newpage
\thispagestyle{empty}

\noindent\textbf{Response to the Review Team's Comments}

\vspace{0.5cm}
\input{tois2023ye/Cover/AE}

\vspace{0.3cm}
\input{tois2023ye/Cover/R1}

\vspace{0.3cm}
\input{tois2023ye/Cover/R2}

\vspace{0.3cm}
\input{tois2023ye/Cover/R3}

\vspace{0.3cm}
\input{tois2023ye/Cover/R4}

\newpage
\normalsize


==> Cover/R1.tex <==
% R1 的回复
\noindent\textbf{Responses to R1:}
\vspace{0.1cm}

\vspace{0.2cm}
\textbf{<R1.1>} \textit{It is unclear how the train-val-test separation is designed for the collected EEG signals. Is it separated by time or by participants or just by random. Different separation strategies will be corresponding to different interpretation of the generalizability of the proposed model.}

\textbf{Response:} 
We have compiled a comprehensive overview of the experimental setup for the RF pipeline in Section~\ref{5.0} and added Algorithm~\ref{algorithm:pipeline} to systematically explain the overall RF experimental setups, especially the data-splitting protocols.
At the same time, redundant content has been removed from Sections~\ref{5.1} and Section~\ref{5.2.1} Line~\lineref{R1.4}.

\textbf{Revision:} \textcolor{blue}{Please refer to Section~\ref{5.0} for revisions of the RF experimental setups.}

\vspace{0.2cm}
\textbf{<R1.2>} \textit{In the design of the proposed framework, EEG signals are considered as an input to the model to help with the estimation of the relevance feedback. Will this be a problem in the real-world when the EEG is hard to obtain?}

\textbf{Response:} Thanks for your concerns. 
To provide a clearer understanding of the EEG availability issue, we have revised Section~\ref{6.2} and Section~\ref{2.3}, incorporating further discussions and updating with recent studies that address this challenge.
In Section~\ref{6.2}, we have discussed the recent developments of portable EEG devices and the possibilities of adopting them in real-world information systems.
Currently, wearable EEG devices are applied in tandem with VR technologies~\cite{tauscher2019immersive} and in services catering to the differently-abled~\cite{11chen2022web}. 
In IR-related research, functional information systems utilizing Brain Computer Interface~(BCI) have been developed. 
A notable instance is the work by \citet{11chen2022web}, who crafted a fully operational BCI-integrated search system that eliminates the need for traditional input devices like keyboards and mouse.
As BCIs become more prevalent and cheaper, we believe that their application scenarios in IR will soon emerge. 
Besides directly controlling information systems, we reveal another benefit of BCI for information systems, i.e., RF. 
The closed loop between the user and the system can be built since the system can better understand the user with the RF model. 

On the other hand, our method can be extended to various information systems that need feedback signals to model users' states.
We suggest that brain signals are special ``explicit feedback'', which directly capture brain activities and are more accurate than implicit feedback signals~(e.g., click, and pseudo signals). 
We also reveal the search scenarios which brain signals perform particularly well.
This implies, considering the issues of user privacy, brain signals do not need to be collected indefinitely, but collecting them in certain scenarios can be particularly helpful.

\textbf{Revision:} \textcolor{blue}{Please refer to Section~\ref{2.3} and Section~\ref{6.2} for revisions on the discussions about the EEG availability issue and applications of our research.}

\vspace{0.2cm}
\textbf{<R1.3>} \textit{BM25 is suggested to be a universal baseline for experiments to make the improvement of the proposed method more convincing.}

\textbf{Response: } We add BM25 as our baseline, detailing its document performance in IRF and RRF experiments in Section~\ref{5}. 
Generally, BM25 underperforms both BERT and Sogou (the initial ranking of a commercial search engine) with some exceptions: in the RRF task, the NDCG@5 of BM25 surpasses that of BERT; in the IRF task, the MAP score of BM25 exceeds that of Sogou.
Although existing research underscores the superior performance of BERT over BM25~\cite{53nogueira2019passage}, the divergence in their performance becomes notably minimal when juxtaposed with the impact of integrating additional feedback information, especially brain signals. 
This suggests that, compared to the incorporation of additional feedback information, particularly brain signals, the impact of selecting text-based ranking models is relatively minimal.

\textbf{Revision:} \textcolor{blue}{Please refer to Table~\ref{tab:irf} and Table~\ref{tab:rrf} for the document ranking performance of BM25 and Section~\ref{5.3} for the analyses of the BM25 performance.}

\vspace{0.2cm}
\textbf{<R1.4>} \textit{Before mentioning “MAP” in the paper, it is suggested to include the full definition of MAP in the paper to make the paper self-contained.}

\textbf{Response:} We add the full definition and reference of MAP in our manuscripts.

\textbf{Revision:} \textcolor{blue}{Please refer to Section~\ref{5.2.1}.}

==> Cover/R2.tex <==
\noindent\textbf{Responses to R2:}
\vspace{0.1cm}

\vspace{0.2cm}
\textbf{<R2.1>} \textit{Brain signal is a kind of user privacy. Users may not intend to share this information, hindering the application of the proposed method.}

\textbf{Response: } Thanks for your comments.
We fully acknowledge the importance of privacy and the balance of technological advancements and ethical considerations. 
We believe that this issue can be mitigated with the advancement of technologies like edge computing, where users have the right to decide whether to upload data to the cloud. 
Other than these methods, according to our experiment results, there are several characteristics of our method that could help it reduce the risk of privacy-related issues in practice: 
(1)~Our model trained with cross-subject data also exhibits good performance, which means that, we may be able to avoid using user's personal data by training and deploying a global brain signal model for everyone while keeping a reasonable retrieval performance.
(2)~Our model trained with a small amount of training data still performs well in the experiments, which means that, in practice, we just need to collect a limited amount of user data to train the model, and then deploy the model to user's device to avoid further collection of user's personal data. 
(3)~Also, as shown in our experiments, the benefits of brain-based relevance feedback are usually observed when users are doing complicated search tasks, especially when conventional user signals are biased. 
Since there are already studies on how to identify task complexity~\cite{arguello2014predicting}, we could use an offline task difficulty classifier to distinguish simple tasks from difficult tasks so that we can collect user data and use our model only when the task is difficult.

To clarify this issue, we add the discussion on (1) and (2) in Section~\ref{5.1}. 
We also shed light on (1),(2), and (3) in Section~\ref{5.3}, and discuss the availability issue and applications of our research in Section~\ref{6.2}.

\textbf{Revision:} \textcolor{blue}{Please refer to Section~\ref{5.1} for the EEG experiments which involves the discussions. 
Kindly refer to Section~\ref{6.2} for discussions about the EEG availability issue and applications of our research. }

\textbf{<R2.2>} \textit{The reviewer noticed there are only 21 participants engaged in this experiment. Have you collected enough data to conduct this experiment? Do your setting and task similar to previous studies?}

\textbf{Response:} Thanks for your concerns. 
In Section~\ref{3.1}, we have addressed the number of participants is analogous to prior EEG-based studies~(e.g.,
18~\cite{76zhang2018relevance} and 23~\cite{57rocchio1971relevance}). 
To address concerns about the number of participants, we add the power analysis result to avoid the risk of Type II errors. 
The estimated sample size for the feature analysis in Section~\ref{5.1} is 18~(statistical power=0.8, $\alpha$=0.05).
This indicates that the number of participants is enough for study the effect of brain signals.


\textbf{Revision:} \textcolor{blue}{
We highlight the relevant description in the revised version in Section~\ref{3.1} Line~\lineref{l3.1}. 
We also provide the result of the statistical power analyses in Section~\ref{3.1} Line~\lineref{l3.1} to address the concerns about the number of participants.
}

\textbf{<R2.3>} \textit{The authors can further clarify the motivation for exploiting brain signals to improve search tasks. Some illustrated examples are expected.}

\textbf{Response: } Thanks for your concerns. We clarify the motivation of exploiting brain signals to improve search tasks in Section~\ref{1} and Section~\ref{6.2}, which is detailed in <AE.3>. We also add a case study in Section~\ref{Case studies} to illustrate the necessity of exploiting brain signals to improve search performance.

\textbf{Revision:} \textcolor{blue}{Please refer to Section~\ref{2.3}, and Section~\ref{6.2} to the discussions of motivations. Please refer to Section~\ref{Case studies} with illustrated examples showing how brain signals benefit search performance.}
 
\vspace{0.2cm}
\textbf{<R2.4>} \textit{This study does not consider the confounding factors that may affect the experimental conclusions, as the causality-related studies show.}

\textbf{Response:} Thank you for your concerns. 
In the data collection procedures, we randomized the task order and the order of the search documents, minimizing the risk of potential confounders. 
However, I concur with your point that incorporating a causality effect analysis can enhance the robustness of the research since it is impossible to completely avoid the effect of all the confounding factors. 
The experimental results in our paper encompass two aspects: (1)~experiments on predicting document relevance using brain signals, and (2)~experiments on RF through the integration of multiple signals.
For (2), the RF performance solely concerns the quality of the brain-based relevance estimation. 
Therefore, we conduct an additional statistical analysis for (1) considering your insightful advice, which can be found in Section~\ref{A.2}.
Following existing literature~\cite{72ye2022don}, the confounding factors we studied include individual differences, the display type of the documents, the task rank, the documents rank, and the word number in the documents.
The experimental results show that the relevance of documents has a significant and detectable effect on participants' brain signals.  
On the other hand, we acknowledge that our research has limitations as we sourced queries exclusively from TREC and iMine, which could introduce confounding factors related to search tasks.
Such queries tend to be concise, cover broad topics, and are relatively easy for detecting the RF effect~\cite{4azad2019query}. 
Therefore, while they serve as a starting point for investigating the influence of brain signals on typical queries, it would be valuable to explore the RF effect under more real-world search tasks, including non-query-based contexts like conversational search.

\textbf{Revision:} \textcolor{blue}{Please refer to Section~\ref{A.2} and Section~\ref{6.3} for the causality-related analyses and discussion on limitations, respectively.}









==> Cover/R3.tex <==
\noindent\textbf{Responses to R3:}
\vspace{0.1cm}

\vspace{0.2cm}
\textbf{<R3.1>} \textit{The main task procedure described in the user study~(Section 3.3) is fairly brief and not very easy to follow. 
It is suggested to provide more examples and screenshots for tasks S1-S4 on top of the one demonstrated in Fig.1 - e.g., by utilizing an appendix.}

\textbf{Response: } Thanks for your comments.
We provide more examples and screenshots to depict the procedures of the main task in Section~\ref{Interface of the lab study} and Figure~\ref{fig:interface}.
We also clarify the presentation Section~\ref{3} to better describe the procedures of the user experiments.
We also update our github with the code and instructions of the user study system for better replication.

\textbf{Revision:} \textcolor{blue}{Please refer to Section~\ref{Interface of the lab study} and Section~\ref{3} for the clarification of the user study procedures.}

\vspace{0.2cm}
\textbf{<R3.2>} \textit{In Section 3.4, although it is understood that the preprocessing of EEG signals follows the practices in existing literature, it is expected to further discuss the sensitivity of the IR model to the EEG data processing protocol, e.g., the high- and low-pass filtering bounds and downsampling rate.}

\textbf{Response: } Thanks for your comments.
We add a sensitivity analysis regarding the data-preprocessing of EEG signals in Section~\ref{Sensitivity analysis}.
The EEG data processing protocol includes data segmentation, high- and low-pass filtering, and down-sampling.
For data segmentation, a duration of 2,000 ms has been identified as a sufficient timeframe to discern human perception concerning relevance, corroborated by previous studies~(\cite{3allegretti2015relevance} and \cite{72ye2022don}) which reported a relevant timeframe of 800 ms. 
The sensitivity analysis also indicates that as the time duration increases, the relevance estimation performance improves, stabilizing between 1,600 ms to 2,000 ms, as depicted in Figure~\ref{fig:time_window}.
For the high- and low-pass filtering bounds we select~(i.e., 0.5 Hz and 50 Hz) are common practice because the range of frequencies produced by the human scalp is between 0.5 and 50 Hz.
Hence, discarding electrical signals outside this range can eliminate the effects of irrelevant electrical signals, such as environmental electricity and electromyography.
For the down-sampling, the sensitivity analysis shows that the relevance estimation performance benefits from limited down-sampling.
For computational efficiency, especially in real-time relevance feedback scenarios, we selected a 500Hz down-sampling rate. This approach yields a performance nearly equivalent to without down-sampling, but is more computationally efficient.

\textbf{Revision:} \textcolor{blue}{Please refer to Section~\ref{Sensitivity analysis} for the sensitivity analysis.}

\vspace{0.2cm}
\textbf{<R3.3>} \textit{The presentation needs to be substantially improved to eliminate syntax and grammatical errors.}

\textbf{Response: } Thanks for the comments. We revised all the issues you noted and polished the paper to improve its readability.

\vspace{0.2cm}
\textbf{<R3.4>} \textit{In the IR method design, the pseudo relevance and click-based relevance both follow the common practice in existing research, while the main highlight is supposed to be the modeling of the brain-based relevance score. However, this part of the design is currently not well-structured and formulated, making the EEG-based relevance score less intuitive and not easy to follow.}

\textbf{Response:} Thank you for your valuable feedback regarding our IR method design, specifically the modeling of EEG-based relevance scores. 
We clarify the EEG-based relevance score modeling in Section~\ref{Brain-based relevance score}, and we add Algorithm~\ref{algorithm:pipeline} to indicate the process of real-time modeling and real-time prediction using EEG.
We also include practical examples to demonstrate the application of EEG-based relevance scores in comparison with traditional RF signals in Section~\ref{Case studies}.

\textbf{Revision:} \textcolor{blue}{Please refer to Section~\ref{Brain-based relevance score} and Section~\ref{5.0} for the clarification of EEG-based relevance score modeling.}

\vspace{0.2cm}
\textbf{<R3.5>} \textit{In line 36 page 17, RRF yields the best results when $\theta^{re,p}$ is set to 0, meaning there is no contribution from the pseudo relevance. It can be discussed further why is this the case, and whether or not it is specific to the experiment data in use.}

\textbf{Response:} Thanks for your concerns. 
We check the experimental codes and confirm that RRF yields the best results when $\theta^{re,p}$ is set to 0 when selected from $\{0,0.2,0.4,0.6,0.8,1.0\}$.
We further search in the 0-0.2 range and observe that the performance of $F_{\Theta^{re}}(R^{bs}, R^c, R^p)$ yields no significant difference in the range of 0-0.14~(peaks at 0.06).
However, the performance of $BERT(R^p)$ is significantly higher than ranking the documents randomly with $p < 0.001$. 
This indicates that pseudo relevance is effective for RRF, but when compared to the user signals~($R^c$ and $R^{bs}$), the effect is very small. 
We speculate that the reasons are:
The documents are selected from top documents while submitting the query to the Sogou's search engine, as explained in Section~\ref{Stimuli Prepartion}.
Therefore, most of them are already semantically related to the query term and their semantic relevance to the query is similar, which is pseudo-relevance measures.
As the queries in our tasks are short and with broad topics,  knowing what topics the user needs is more important than the little differences in semantic relevance.
Hence, the effect of pseudo-relevance is minimal when compared to the user signals. 

We admit that this is related to the experiment data as the queries are selected from TREC and iMine, which tend to be concise, cover broad topics, and are relatively easy for detecting the RF effect~\cite{4azad2019query}. 
We clarify this issue in Section~\ref{5.2} and polish the discussion about this selection bias in Section~\ref{6.3}.
% In the era of neural ranking~(e.g., BERT-based methods), due to the ability to represent queries as a semantic vector rather than ``bag of words'', the problem of term-mismatch has been greatly alleviated, and the need for pseudo-relevance feedback is not as significant as before.

\textbf{Revision:} \textcolor{blue}{For discussion on the minimal impact of pseudo-relevance, please refer to Section~\ref{5.2} Line~\lineref{R3.5}. Please refer to Section~\ref{6.3} for the discussion of limitations.}

\vspace{0.2cm}
\textbf{<R3.6>} \textit{In Section 5.3, it should be clarified how are the ``ideal'' combination coefficients are obtained, including the search space and search method.}

\textbf{Response:} Thanks for your comments. 
We clarify the process of obtaining the ``ideal'' combination coefficients in Section~\ref{5.3}. 
For every data sample, we search values for $\theta^{,\dagger}$, where $ \in {it, re}$ and $\dagger \in {bs, c, p}$, from the set ${0.0, 0.2, 0.4, 0.6, 0.8, 1.0}$, i.e., the same search space as detailed in the experimental setup~(see in Section~\ref{5.2}). 
Subsequently, we determine the optimal combination of parameters $\Theta^{it}$ and $\Theta^{re}$ based on the NDCG@10 for each distinct data sample.

\textbf{Revision:} \textcolor{blue}{Please refer to Section~\ref{5.3} Line~\ref{R3.6} for the clarification.}

\vspace{0.2cm}
\textbf{<R3.7>} \textit{This paper should be concluded with more actionable insights w.r.t. this line of research. Specifically, what are recommended practices for designing the human study, data collection, and data preprocessing protocols? Is it possible to train, or fine-tune a neural ranker with a limited amount of BCI signals on complex tasks given the current difficulty for such data collection to scale? Is the integration of BCI signals able to resolve some long-standing research IR questions such as exposure/popularity/presentation bias and query evaluation?}

\textbf{Response:} Thanks for your valuable comments. 
We add the actionable insights regarding our research in Section~\ref{6.2} and discussion with previous work in Section~\ref{2.3}.
Specifically, we provide responses to the points of concern as follows: 
\begin{itemize}
    \item \textbf{Response to the recommended practices for designing the human study \& limited amount of BCI signals on complex tasks:} 
    In our study, we aimed to implement settings that closely resemble real-world scenarios. 
    For instance, instead of using random data splitting as done in prior research, we adopted a split-by-timepoint splitting to simulate the cold start situation that new users experience when they begin using our system. 
    Our findings indicate that using a general model during the cold start phase and training a subject-specific model during the search process can yield practicable results. 
    Furthermore, we conducted sensitivity analyses to demonstrate the impact of EEG preprocessing methods on relevance prediction.
    \item \textbf{Response to solving long-standing research IR questions:} 
    Since traditional interaction paradigms can only capture indirect user feedback, biases in these behaviors have been long-standing IR research problems.
    To address these challenges, we propose utilizing brain signals as a unique form of ``explicit feedback''.
    Concurrently, we identify specific search scenarios in which biases in user behaviors may adversely affect RF performance, highlighting instances where brain signals can offer significant advantages.
    We recognize the significance of exposure/presentation biases in IR. 
    However, addressing these biases is beyond the purview of this paper. 
    Because if a document isn't presented or exposed to the user, we cannot obtain their brain responses to it either.
\end{itemize}

\textbf{Revision:} \textcolor{blue}{Please refer to Section~\ref{6.2} regarding our research insights and Section~\ref{2.3} for comparison with previous work.}



==> Cover/R4.tex <==
\noindent\textbf{Responses to R4:}
\vspace{0.1cm}

\vspace{0.2cm}
\textbf{<R4.1>} \textit{Compared to brain signals, eye movement may be easier to track and used to give feedback on which results are interested by a user. Have authors considered using such kind of signals?}

\textbf{Response:} Thanks for your concerns. 
The utilization of eye movement tracking is indeed a compelling approach, given its potentially more accessible nature than brain signals.
However, existing research has shown that eye-tracking and mouse movements are not accurate enough since they are also indirect probes of user signals~\cite{mao2014estimating}.
The main difference between brain signals and the aforementioned signals is that brain signals provide direct feedback on a person's consciousness and thoughts, thus avoiding the biases associated with behavioral signals. 
The only concern lies in the noise introduced during brain signal collection and decoding, which can be further mitigated through improved equipment and data quality.
In our study, we only compare brain signals with pseudo-relevance signals and click signals.
However, the idea of integrating eye movement data or even comparing both modalities in a future investigation is intriguing and holds merit. 
We acknowledge the valuable feedback and will certainly consider the potential of eye movement tracking in enhancing the methodology and findings of subsequent studies on this topic.

\textbf{Revision:} \textcolor{blue}{Please refer to Section~\ref{6.2} and Section~\ref{2.3} for the comparison of eye-tracking techniques and brain techniques and Section~\ref{6.3} for our limitation and future work.}

\vspace{0.2cm}
\textbf{<R4.2>} \textit{There is still room to improve on presentation.}

\textbf{Response:} Thanks for the comments. We revised all issues you noted~(Line~\lineref{R4.2.0},  \lineref{R4.2.1}, \lineref{R4.2.2}, \lineref{R4.2.3}, \lineref{R4.2.5}, and \lineref{R4.2.7}) and polish the whole paper to fix syntax error and improve its readability.


==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> meta/case_study.tex <==
\newlength{\dlength}
% 设置长度 x 的值为 3cm
\setlength{\dlength}{3.3cm}
\begin{table}[]
\begin{tabular}{|p{\dlength}p{\dlength}|lll|ll|ll|}
\hline
\multicolumn{2}{|c|}{\textbf{Query:  The Prophet}} & \multicolumn{3}{l|}{\textbf{Base scores}} & \multicolumn{2}{l|}{\textbf{IRF}} & \multicolumn{2}{l|}{\textbf{RRF}} \\ \hline
\multicolumn{1}{|p{\dlength}|}{\makecell[c]{Historical documents \\ ($D^h$)}}& \makecell[c]{Unseen documents \\ ($D^u$)} & \multicolumn{1}{l|}{$R^c$} & \multicolumn{1}{l|}{$R^p$} & $R^{bs}$ & \multicolumn{1}{l|}{\makecell[c]{w \\ $R^{bs}$}} & \makecell[c]{w/o \\ $R^{bs}$} & \multicolumn{1}{l|}{\makecell[c]{w \\ $R^{bs}$}} & \makecell[c]{w/o \\ $R^{bs}$} \\ \hline
\multicolumn{1}{|p{\dlength}|}{d1: The Prophet - French, rough, crime}             & d7: Analysis and translation of the Prophet's poem  & \multicolumn{1}{l|}{\makecell[c]{d1:\\0}}              & \multicolumn{1}{l|}{\makecell[c]{d1:\\0.6}}               &            \makecell[c]{d1: \\ 0.3}                 & \multicolumn{1}{l|}{\textcolor{blue}{d11}} & \textcolor{blue}{d11} & \multicolumn{1}{l|}{\textcolor{blue}{d4}} & \textcolor{blue}{d6} \\ \hline
\multicolumn{1}{|p{\dlength}|}{\textcolor{lightblue}{d2: Miracles of the Mohammed Prophet}}  & \textcolor{lightblue}{d8: What does the prophet mean in the Bible? - Sogou ask}                & \multicolumn{1}{l|}{\makecell[c]{\textcolor{lightblue}{d2:}\\0}}              & \multicolumn{1}{l|}{\makecell[c]{\textcolor{lightblue}{d2:}\\0.2}}               &               \makecell[c]{\textcolor{lightblue}{d2:}\\0.6}              & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{\textcolor{blue}{d6}} & \textcolor{blue}{d4} \\ \hline
\multicolumn{1}{|p{\dlength}|}{d3: The Prophet poem by Gibran} & d9:  The Prophet movie: free  online resource & \multicolumn{1}{l|}{\makecell[c]{d3:\\0}}& \multicolumn{1}{l|}{\makecell[c]{d3:\\0.3}}& \makecell[c]{d3:\\0.3} & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{\textcolor{lightblue}{d2}} & d1 \\ \hline
\multicolumn{1}{|p{\dlength}|}{\textcolor{blue}{d4: The Prophet - Sogou encyclopedia}}  & d10: \textit{The Prophet} : Gibran & \multicolumn{1}{l|}{\makecell[c]{\textcolor{blue}{d4:}\\1}} & \multicolumn{1}{l|}{\makecell[c]{\textcolor{blue}{d4:}\\0.3}}   &  \makecell[c]{\textcolor{blue}{d4:}\\0.7}                           & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{d1} &  d3\\ \hline
\multicolumn{1}{|p{\dlength}|}{d5: Fifth personality -   introduction of the Prophet} & \textcolor{blue}{d11: The Prophet in different cultures}               & \multicolumn{1}{l|}{\makecell[c]{d5:\\0}}              & \multicolumn{1}{l|}{\makecell[c]{d5:\\0.2}}               &       \makecell[c]{d5:\\0.2}                      & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{d3} & \textcolor{lightblue}{d2} \\ \hline
\multicolumn{1}{|p{\dlength}|}{\textcolor{blue}{d6: General concepts of ``Prophet''}}           &  \textcolor{lightblue}{d12:  The Prophet - Chinese dictionary}                  & \multicolumn{1}{l|}{\makecell[c]{\textcolor{blue}{d6:}\\1}}              & \multicolumn{1}{l|}{\makecell[c]{\textcolor{blue}{d6:}\\0.4}}               &   \makecell[c]{\textcolor{blue}{d6:}\\0.6}                          & \multicolumn{1}{l|}{} &  & \multicolumn{1}{l|}{d5} & d5 \\ \hline
\end{tabular}
\caption{Case study}
\label{tab:case_study}
\end{table}









